FairDiffusion: Enhancing Equity in Latent Diffusion Models via Fair Bayesian Perturbation

Recent progress in generative AI, especially diffusion models, has demonstrated significant utility in text-to-image synthesis. Particularly in healthcare, these models offer immense potential in generating synthetic datasets and training medical students. However, despite these strong performances, it remains uncertain if the image generation quality is consistent across different demographic subgroups. To address this critical concern, we present the first comprehensive study on the fairness of medical text-to-image diffusion models. Our extensive evaluations of the popular Stable Diffusion model reveal significant disparities across gender, race, and ethnicity. To mitigate these biases, we introduce FairDiffusion, an equity-aware latent diffusion model that enhances fairness in both image generation quality as well as the semantic correlation of clinical features. In addition, we also design and curate FairGenMed, the first dataset for studying the fairness of medical generative models. Complementing this effort, we further evaluate FairDiffusion on two widely-used external medical datasets: HAM10000 (dermatoscopic images) and CheXpert (chest X-rays) to demonstrate FairDiffusion's effectiveness in addressing fairness concerns across diverse medical imaging modalities. Together, FairDiffusion and FairGenMed significantly advance research in fair generative learning, promoting equitable benefits of generative AI in healthcare.

==> sec/conclusion.tex <==
% \section{Conclusion}
% We present the first comprehensive study investigating the fairness of medical text-to-image diffusion models. Our extensive evaluations of the widely used Stable Diffusion model reveal significant disparities across all protected attributes in both the generation and classification settings. To address these fairness gaps, we propose FairDiffusion, an equity-aware generative learning model that improves both overall performance and fairness. Moreover, we also introduce FairGenMed, the first dataset for studying fairness of medical generative models. To aid future research in fair generative learning, we make our code and dataset publicly available.

==> sec/related.tex <==
% \section{Related Work}

% \noindent\textbf{Image Synthesis Techniques}.
% Image synthesis (or image generation) is a longstanding research problem that aims to artificially generate images that contain some particular desired content \cite{Shimoda1989New,Wandell1992The}. Prior-art techniques that tackle this problem include Variational Autoencoders (VAEs) \cite{kingma2013auto,kingma2019introduction} and Generative Adversarial Networks (GANs) \cite{goodfellow2014generative,liu2016coupled,karras2019style,zhang2019self}. VAEs suffer from posterior collapse \cite{wang2021posterior}, while GANs face challenges like mode collapse \cite{srivastava2017veegan}. In contrast, physics-inspired diffusion models recently rising show that better stable trainability than VAEs and GANs \cite{sohl2015deep,ho2020denoising,rombach2022high}. Specifically, Rombach \etal, propose a guiding mechanism to control image generation without retraining and introduces cross-attention layers to enhance the model's flexibility for conditioning inputs like text or bounding boxes \cite{rombach2022high}.
% Podell \etal, further enhance the Stable Diffusion \cite{rombach2022high} by utilizing a three times larger UNet backbone, achieved through an increase in attention blocks and a larger cross-attention context with the incorporation of a second text encoder \cite{podell2024sdxl}. Stable diffusion models can also extend to video generation tasks \cite{yu2023video}. 

% % \begin{table}[!t]
% % 	\centering
% %     % \vspace{-10mm}
% % 	% \caption{\label{tbl:dataset}
% % 	%    Public medical fairness datasets. Note that the text in CheXpert/MIMIC-CXR is radiology report authored by radiologists, which centers around the corresponding image. In the case of FairVLMed, the text is clinical note authored by doctors, which centers around the patient and their specific medical condition.
% % 	% }
% % 	\caption{\label{tbl:dataset}
% % 	Public medical fairness datasets (comparison). In contrast to existing medical VL datasets, FairVLMed provides detailed demographic attributes, ground-truth labels, and clinical notes with imaging as well as non-imaging clinical information.  
% % 	}
% %         % \vspace{-1ex}
% % 	\adjustbox{width=1\columnwidth}{
% % 	\begin{tabular}{ L{20ex} L{18ex} L{12ex} L{12ex} L{18ex} C{7ex} L{15ex}}
% % 		\toprule
% % 		\textbf{Dataset} & \textbf{Disease} & \textbf{\# of Images} & \textbf{\# of Patients}  & \textbf{Protected Attribute} & \textbf{Align} & \textbf{Clinical Measurement}\\

% % \cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5} \cmidrule(lr){6-6} \cmidrule(lr){7-7} 



% % Fitzpatrick17k \cite{groh2021evaluating}  & Dermatological Disease  & 16,012  & 1,373 & Skin type  & \xmark & - \\

% % HAM10000 \cite{tschandl2018ham10000} & Dermoscopical Disease & 9,948  & - & Age; Gender & \cmark & -\\
% % %OpenPath \cite{huang2023visual} & pathology image-text pairs from twitter/internet/LAION-dataset & 208,414 & N/A & N/A & \cmark & \cmark & Image Description\\

% % OL3I\cite{zambrano2021opportunistic} & Heart Disease & 8,139   & 1,686 & Age; Gender  & \cmark & -\\
% % ODIR-2019 \cite{odir2019} & Ocular Disease & 8,000  & 5,000  & Age; Gender  & - & -\\
% % PAPILA \cite{kovalyk2022papila} & Glaucoma & 488  &  244 & Age; Gender  & - & -\\

% % Harvard-GDP \cite{Luo_2023_ICCV} & Glaucoma and OCT & 1,000 & 1,000 & Age; Gender; Race & \xmark & \\
% %    %\cmidrule(lr){1-8}
% % COVID-CT-MD\cite{afshar2021covid} & Pneumonia & 308 & 305 & Age; Gender & \cmark & -\\

% % AMD-OCT\cite{farsiu2014quantitative} & AMD & 384 & - & Age  & - & -\\

% % ADNI 1.5T \cite{wyman2013standardization} & Alzheimer's Disease & 550 & & Age; Gender & \cmark & - \\

% %    % \cmidrule(lr){1-7}

% %    CheXpert \cite{irvin2019chexpert} & Chest Disease & 222,793   & 65,240 & Age; Gender; Race & \cmark & -\\

% % MIMIC-CXR \cite{Johnson_arXiv_2019} & Chest Disease & 370,955  &  65,079 & Age; Gender; Race & \cmark & - \\
% % PadChest \cite{bustos2020padchest} & Chest Disease & 160,868  & 69,882 & Age; Gender & \cmark & -\\

% % GlaucomaFairness \cite{luo2023harvard} & Glaucoma & 3,300 & 3,300 & Age; Gender; Race; Ethnicity; Preferred Language; Marital Status & \xmark & - \\

% % FairSeg \cite{tian2024fairseg} & Glaucoma & 10,000 & 10,000 & Age; Gender; Race; Ethnicity; Preferred Language; Marital Status & \xmark & Disc and Cup Borders \\

% % EyeFairness \cite{tian2024fairseg} & AMD; DR; Glaucoma & 30,000 & 30,000 & Age; Gender; Race; Ethnicity; Preferred Language; Marital Status & \xmark & - \\

% % FairGenMed  & Glaucoma & 10,000 & 10,000 & Age; Gender; Race; Ethnicity; Preferred Language; Marital Status & \cmark & Vision Loss Severity; Cup-Disc Ratio Status; Spherical Equivalent Status \\

% % % FairVLMed & Glaucoma & 10,000 & 10,000 & Age; Gender; Race; Ethnicity; Preferred Language; Marital Status & \cmark & - \\


% % 		\bottomrule	
% % 	\end{tabular}}
% %  % \vspace{-7 mm}
% % \end{table}

% \noindent\textbf{Datasets for Fairness Learning}.
% Fairness studies in medical imaging highlight the significance of having diverse and representative datasets. This section reviews datasets that advance the study of fairness within the medical domain. Specifically, in dermatology, the Fitzpatrick17k \cite{groh2021evaluating} and HAM10000 \cite{tschandl2018ham10000} datasets offer data across sensitive attributes, including various skin types, age groups, and genders. In the cardiology domain, the OL3I dataset \cite{zambrano2021opportunistic} provides heart CT data across age and gender demographics. In the context of chest x-ray analysis, the CheXpert \cite{irvin2019chexpert}, MIMIC-CXR \cite{Johnson_arXiv_2019}, COVID-CT-MD\cite{afshar2021covid} and PadChest \cite{bustos2020padchest} datasets provide chest radiographs accompanied by demographic information like age, gender, and race. The inclusion of these attributes is essential for assessing and mitigating potential biases in models trained for diagnosing chest diseases.

% Similarly, in the field of ophthalmology, datasets such as ODIR-2019 \cite{odir2019} and PAPILA \cite{kovalyk2022papila} provide insights into ocular conditions across various age groups and genders. Moreover, the introduction of Harvard-GDP \cite{Luo_2023_ICCV}, GlaucomaFairness \cite{luo2023harvard}, FairSeg \cite{tian2024fairseg} and EyeFairness \cite{tian2024fairseg} further advances fairness research in ophthalmology, particularly in fair glaucoma detection, by including detailed demographic attributes, encompassing age, gender, race, ethnicity, preferred language and socioeconomic factors. In particular, FairSeg \cite{tian2024fairseg} also provides additional clinical measurements such disc and cup borders enhancing its utility in specialized medical evaluations. 

% Although the aforementioned datasets have advanced fairness studies within medical imaging, they have not specifically addressed generative tasks. Given the growing interest in generative models, we introduce FairGenMed, a novel dataset tailored for assessing fairness in medical generative models. Unlike existing datasets, which face challenges in fairness analysis due to noisy labels from automated extraction processes, FairGenMed provides precise ground-truth labels alongside quantitative clinical measurements such as cup-disc ratio (CDR), retinal nerve fiber layer thickness (RNFLT), and spherical equivalent (SE) refractive error. Amidst the surging interest in generative models, FairGenMed can serve as a key resource to catalyze developments in creating more equitable and unbiased generative learning algorithms.



% \noindent\textbf{Bayesian Optimization}. Bayesian optimization is a strategy for efficiently optimizing black-box functions, which uses a probabilistic model, commonly instantiated as a Gaussian Process, to balance exploration and exploitation based on observed data. The method iteratively updates this model via Bayesian inference, guiding the selection of subsequent evaluation points to minimize the number of function evaluations. Bayesian optimization was first introduced by Harold Kushner~\cite{kushner1964new}, who employed Wiener processes to solve unconstrained one-dimensional optimization problems, aiming to maximize the probability of selecting samples that would lead to improvements. This approach was further developed by researchers~\cite{stuckman1988global,perttunen1990rank,elder1992global}, extending its application to high-dimensional optimization challenges and significantly broadening its utility. Building upon this foundational work, Mockus~\cite{movckus1975bayesian} introduced the expectation of improvement as a novel acquisition function. In contrast, the upper confidence bound (UCB) method balances exploration and exploitation by considering uncertainty \cite{williams2006gaussian}. In this work, we employ the Bayesian Optimization technique to adaptively perturb the learning process to enhance equity in the image generation task.
% % Subsequently, some studies~\cite{van2003kriging,huang2006global} have focused on refining this optimization strategy to accommodate constraints and noise within the optimization process, thereby enhancing its effectiveness and adaptability for more complex optimization scenarios.

==> sec_revision/dataset.tex <==
\section{Dataset Analysis}
This study rigorously follows the principles delineated in the Declaration of Helsinki and has obtained approval from our institute's Institutional Review Board. All data within this dataset have been de-identified.

% \subsection{Data Collection and Quality Control}

% The subjects who received glaucoma services between 2015 and 2022 were sourced from a large academic eye hospital. This study is based on scanning laser ophthalmoscopy (SLO) fundus images, which serve as a valuable marker for assessing retinal damage. The dataset includes multiple protected identity attributes, such as age, gender, race, ethnicity, preferred language, and marital status, associated with each SLO fundus image. we de-identify SLO fundus images to ensure that there is no identifying information on the images. 

% Subjects are categorized into non-glaucoma and glaucoma based on their visual function assessed through visual field (VF) testing. The severity of a medical condition can be further categorized based on certain clinical measurements. For instance, the mean deviation (MD) of visual field is categorized as severe if it's less than -12 dB, moderate if it's between -12 dB and -6 dB, mild if it's between -6 dB and -1 dB, and normal otherwise. Similarly, the cup-to-disc ratio (CDR) is considered abnormal if it's greater than or equal to 0.7, borderline if it's between 0.6 and 0.7, and normal otherwise. Lastly, the near vision refraction stage is classified as negative if it's less than or equal to -0.5 diopters, neutral if it's between -0.5 and 0.5 diopters, and positive otherwise.


% \revise{\sout{\subsection{Data Characteristics}}}
The FairGenMed dataset comprises 10,000 samples from 10,000 subjects. It is divided into 6,000 training, 1,000 validation, and 3,000 test samples.
The dataset's average age is 61.6 $\pm$ 15.6 years. The dataset includes samples from three major groups: Asian, with 819 samples; Black, with 1,491 samples; White, with 7,690 samples. The dataset also includes two gender categories: Female and Male, with 5824 and 4176 individuals, respectively. In terms of ethnicity, there are two categories: Hispanic and non-Hispanic, with 9622 and 378 individuals, respectively. 

Regarding clinical measurements, as shown in Fig. \ref{fig:stats}, the cup-to-disc ratio is categorized as abnormal, borderline, or normal, with 3,067, 2,884, and 4,049 individuals, respectively. Moreover, the vision loss severity is categorized as mild, moderate, normal, or severe, with 2,143, 1,475, 4,994, and 1,388 individuals, respectively. Lastly, the near vision refraction stage is categorized as negative, neutral, or positive, with 926, 7,946, and 1,078 individuals, respectively. This information can be useful for analyzing the prevalence and distribution of various ocular conditions in the dataset.

% There are three racial categories: Asian, Black, and White, with 827, 1448, and 7725 individuals, respectively. The dataset also includes two gender categories: Female and Male, with 5824 and 4176 individuals, respectively. In terms of ethnicity, there are two categories: Hispanic and non-Hispanic, with 9622 and 378 individuals, respectively. 

% The ethnic distribution is highlighted by 90.6\% Non-Hispanic, 4.0\% Hispanic, and 5.4\% unspecified. In terms of preferred language, 92.5\% of the subjects prefer English, 1.7\% prefer Spanish, 0.8\% prefer other languages, and 5.0\% remain unknown. From a marital status perspective, 57.4\% are in a marriage or partnered, 26.4\% are single, 6.6\% have experienced divorce, 1.0\% are legally separated, 6.1\% are widowed, and 2.5\% are not specified. After de-identification, clinical notes vary from 11 to 332 words, with an average word count of 147.

==> sec_revision/intro.tex <==
\section{Introduction}
Generative modeling has witnessed rapid progress, powered largely by advancements in diffusion models in recent years.
Diffusion models \cite{ho2020denoising,sohl2015deep} are used as powerful tools in various scientific fields, offering innovative approaches to complex problems, such like protein structure discovery \cite{wu2024protein}, quantum circuit synthesis \cite{furrutter2024quantum}, peptide conformational sampling \cite{abdin2024direct}, molecular linker design \cite{igashov2024equivariant}, or embodied artificial agents \cite{berrueta2024maximum}.
Specifically, text-to-image diffusion models like Stable Diffusion~\cite{rombach2022high} have demonstrated significant utility across a wide range of different domains. This text-conditioned generative modeling is especially useful in the medical domain, where it offers immense potential in generating synthetic datasets and training medical students to understand different conditions (e.g., eye diseases). Via leveraging advanced image synthesis methods\revise{~\cite{pinaya2022brain,packhauser2023generation,madani2018chest,shah2022dc,motamed2021data,malygina2019data,karbhari2021generation,srivastav2021improved,moris2022unsupervised, song2021solving, xie2022measurement, chung2022score, hu2022unsupervised, ozbey2023unsupervised}}%Diffusion: ~\cite{chambon2022adapting,chambon2022roentgen,khader2022medical,pinaya2022brain,packhauser2023generation,madani2018chest,shah2022dc,motamed2021data,malygina2019data,karbhari2021generation,srivastav2021improved,moris2022unsupervised}
, medical educators can create highly realistic and diverse datasets of various eye disease conditions. These synthesized images can accurately represent a wide range of pathological manifestations, including subtle variations and rare cases that may be challenging to encounter in real-world clinical settings, resulting in more skilled medical practitioners. 


However, despite these strong performances, it remains unclear whether the quality of image generation is consistent across different demographic subgroups. Fairness gaps in image generation quality across different protected attributes raise significant ethical and equity issues, especially in the medical domain where such biases could inadvertently perpetuate healthcare disparities~\revise{\cite{xu2024addressing, tian2025fairdomain, ktena2024generative, drukker2023toward}}. Hence, ensuring fairness in medical image generation is not only a critical challenge from a technical standpoint but also a moral imperative in order to ensure that advances in generative models do not exacerbate existing healthcare inequalities.

To address these critical concerns, we conduct the first comprehensive study on the fairness of medical text-to-image diffusion models. Specifically, using the popular Stable Diffusion~\cite{rombach2022high} model, we conduct two types of fairness evaluations. Firstly, we evaluate the generation quality of the diffusion model across different demographic subgroups. Secondly, we train a classifier with the generated dataset to examine the semantic correlation of clinical features in text prompts with the generated images across various subgroups. Our comprehensive evaluations of the Stable Diffusion model reveal significant biases across all protected attributes in terms of both image generation quality as well as semantic correlation of clinical features. For instance, the Female, White, and non-Hispanic subgroups show improved image generation performance across the protected attributes of gender, race, and ethnicity, whereas the Male, Asian, and non-Hispanic subgroups are favored in the semantic correlation setting on the glaucoma classification task.

To tackle these fairness gaps, we propose FairDiffusion (Fig. \ref{fig:tease_img}), an equity-aware stable diffusion model designed to improve fairness in medical image generation. FairDiffusion employs a Bayesian Optimization based approach and works by adaptively perturbing the learning process with samples from each demographic group in order to achieve fair generative learning. Our proposed FairDiffusion method significantly improves both overall performance and fairness across image generation quality as well as semantic correlation of clinical features. In the image generation quality setting, FairDiffusion leads to notable improvements for the Black and Hispanic subgroups, with \revise{Fréchet Inception Distance (FID)} gains of 7.84 and 11.79 respectively. In the semantic correlation setting, FairDiffusion achieves large gains for the Asian and Male subgroups, with AUC enhancements of 10.03 and 7.58 respectively, on the glaucoma classification task.

In addition to the proposed FairDiffusion method, we also introduce FairGenMed, the first dataset for studying fairness of medical generative models. While existing radiology datasets could be repurposed for fairness analysis, prior works~\cite{seyyed2020chexclusion,irvin2019chexpert} have shown the difficulties of using these datasets for fairness studies. These challenges stem from the automatic extraction of~\textit{ground-truth} labels from radiology reports, potentially resulting in inaccurate fairness assessments due to the noisy labels. In contrast to existing datasets, FairGenMed not only provides ground-truth labels but also includes detailed quantitative measurements of different clinical conditions such as cup-disc ratio (CDR), retinal nerve fiber layer thickness (RNFLT), and near vision refraction (NVR). Since these conditions are naturally correlated with retinal anatomy and pathophysiology, they serve as excellent resources for studying the semantic correlation between text prompts and anatomical regions across various demographic subgroups. With the rapid increase in popularity of generative models, FairDiffusion and FairGenMed have significant potential to drive advancements in equitable and fair generative learning algorithms.

\begin{figure*}[t]
  \centering
    \includegraphics[width=0.6\textwidth]{fig/rebuttal/Figure Final Version cc.pdf}
  \caption{\textbf{a.} General workflow of SLO fundus images generation with generative artificial intelligence (AI) models from text prompt instructions describing clinical features. A carefully designed and curated clinical dataset FairGenMed is used to perform the text-to-image generation task in this study. The generative AI can be potentially used for the purposes of medical education, data sharing, and data augmentation. \textbf{b.} The off-the-shelf generative AI model termed Stable Diffusion model uses clinical features as text prompt input to generate corresponding SLO fundus images.
  % Demographic information is also included in the text prompt to guide the model to generate demographics-aware SLO fundus images.
  \textbf{c.} The FairDiffusion model uses clinical features as text prompt input to generate SLO fundus images with fair Bayesian perturbation to determine demographic group-specific statistical generation parameters. 
  % Leveraging demographic group information in the way of determining group-specific statistical generation parameters instead of using demographics as part of the text prompt allows the generative AI to encode and decode the demographic information more thoroughly.
  \textbf{d.} Contribution 1: FairDiffusion for group-specific statistical generations improves generative AI equity. Contribution 2: Fairness assessment pipeline for medical imaging to quantify the semantic correlations of clinical features between text prompt input and generated SLO fundus images. Contribution 3: A clinical text-to-image fair generation dataset FairGenMed provides a unique dataset for studying fairness issues in generative AI for medical tasks.
  }
  
   \label{fig:tease_img}
 \end{figure*}

\begin{figure*}[t]
  \centering
    \includegraphics[width=1.\textwidth]{fig/nature_machine_intelligence_final_vis.png}
  \caption{Qualitative visualizations of Stable Diffusion and FairDiffusion generated images against real images from the FairGenMed dataset. \revise{Given the images in this figure, FairDiffusion achieves a IS score of 1.5, while Stable Diffusion achieves a IS score of 1.3.}
  }
  \label{fig:qual_vis}
\end{figure*}

